Relative Drawing Identification Complexity is Invariant to Modality in Vision-Language Models

Large language models have become multimodal, and many of them are said to integrate their modalities using common representations. If this were true, a drawing of a car as an image, for instance, should map to a similar area in the latent space as a textual description of the strokes that form the drawing. To explore this in a black-box access regime to these models, we propose the use of machine teaching, a theory that studies the minimal set of examples a teacher needs to choose so that the learner captures the concept. In this paper, we evaluate the complexity of teaching vision-language models a subset of objects in the Quick, Draw! dataset using two presentations: raw images as bitmaps and trace coordinates in TikZ format. The results indicate that image-based representations generally require fewer segments and achieve higher accuracy than coordinate-based representations. But, surprisingly, the teaching size usually ranks concepts similarly across both modalities, even when controlling for (a human proxy of) concept priors, suggesting that the simplicity of concepts may be an inherent property that transcends modality representations.

==> tables/concepts.tex <==
\begin{longtable}{lrrrrrrrr}
\caption{Statistical analysis of the stroke count for each concept.}\label{tab:concepts}\\
\toprule
                Concept &    No. Samples &  AVG &  STD &  Min. &  25\% &   50\% &   75\% &    Max. \\
\midrule
\endfirsthead
\caption[]{Statistical analysis of the stroke count for each concept.} \\
\toprule
                Concept &    No. Samples &  AVG &  STD &  Min. &  25\% &   50\% &   75\% &    Max. \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{{Continued on next page.}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
                   Line & 140874 &   5 &  3.6 &  2 &  3 &   4 &   6 &  186 \\
               Triangle & 120500 &  14.8 &  4.9 &  2 & 12 &  14 &  17 &  222 \\
                 Stairs & 122766 &  14.9 &  6.1 &  2 & 12 &  14 &  16 &  125 \\
                 Square & 120538 &  16.2 &  4.3 &  2 & 14 &  16 &  18 &  181 \\
                Hexagon & 135803 &  16.9 &  4.6 &  2 & 14 &  16 &  19 &  200 \\
               Mountain & 123381 &  17.3 &  6.9 &  2 & 13 &  16 &  21 &  171 \\
                 Zigzag & 116635 &  17.8 &  7.5 &  2 & 13 &  16 &  21 &  138 \\
             Skyscraper & 161800 &  18 & 12.2 &  2 & 12 &  15 &  20 &  220 \\
                    Leg & 110683 &  18.1 &  9.8 &  2 & 11 &  17 &  23 &  256 \\
                   Knee & 245601 &  18.8 &  9.4 &  2 & 13 &  17 &  22 &  213 \\
                  Rifle & 150518 &  19.5 &  8.7 &  2 & 13 &  18 &  24 &  280 \\
              Golf Club & 172882 &  19.8 &  8.9 &  2 & 15 &  18 &  23 &  223 \\
                Octagon & 147718 &  19.9 &  5.5 &  2 & 17 &  19 &  23 &  129 \\
                  Canoe & 119098 &  20 &  9.6 &  2 & 15 &  18 &  22 &  358 \\
                 Ladder & 121605 &  20.4 &  6.9 &  2 & 16 &  19 &  23 &  167 \\
                   Nose & 182477 &  21.1 &  9.1 &  2 & 15 &  20 &  25 &  230 \\
                See Saw & 119586 &  21.1 & 11.9 &  2 & 13 &  18 &  25 &  217 \\
               Keyboard & 165808 &  21.2 & 16.6 &  2 & 14 &  17 &  23 & 1740 \\
           Hockey Stick & 123911 &  21.5 & 11.5 &  2 & 16 &  20 &  24 &  312 \\
                  Knife & 150696 &  21.7 &  8.3 &  2 & 17 &  20 &  25 &  227 \\
                  Bench & 120210 &  21.7 & 12.9 &  2 & 13 &  18 &  27 &  201 \\
                   Tent & 126827 &  21.8 &  8.2 &  2 & 16 &  20 &  25 &  165 \\
                 Finger & 155257 &  22.1 & 10.3 &  2 & 15 &  20 &  26 &  237 \\
              Lightning & 141703 &  22.3 & 13.9 &  2 & 13 &  18 &  27 &  233 \\
              Swing Set & 116404 &  22.7 &  8.6 &  2 & 17 &  21 &  27 &  156 \\
               Stitches & 113995 &  22.8 & 11.1 &  2 & 16 &  20 &  25 &  225 \\
            String Bean &  97166 &  22.9 & 15.4 &  2 & 15 &  18 &  24 &  295 \\
                   Door & 115747 &  23.2 &  8.7 &  2 & 18 &  22 &  27 &  179 \\
               Lipstick & 121264 &  23.3 &  7.9 &  2 & 19 &  22 &  26 &  214 \\
                  Chair & 203526 &  23.3 & 11.3 &  2 & 14 &  22 &  31 &  276 \\
                 Pillow & 111757 &  23.4 &  8.2 &  2 & 18 &  22 &  27 &  152 \\
                  Elbow & 116123 &  23.6 & 12.1 &  2 & 16 &  20 &  29 &  245 \\
                   Fork & 119144 &  23.6 &  9 &  2 & 17 &  22 &  29 &  241 \\
                  Table & 122094 &  23.8 &  8.7 &  2 & 18 &  23 &  28 &  195 \\
                  Spoon & 119918 &  24 &  7.4 &  2 & 20 &  23 &  27 &  330 \\
               Envelope & 130144 &  24 &  6.5 &  2 & 20 &  23 &  27 &  139 \\
                Diamond & 126867 &  24 & 10.4 &  2 & 17 &  22 &  29 &  226 \\
               Suitcase & 121222 &  24 &  9.7 &  2 & 18 &  23 &  28 &  197 \\
            Wine Bottle & 121350 &  24.2 &  7.6 &  2 & 19 &  23 &  27 &  203 \\
            Streetlight & 117417 &  24.3 & 12 &  2 & 16 &  21 &  29 &  179 \\
                  Ocean & 126507 &  24.5 & 15.1 &  2 & 15 &  21 &  29 &  271 \\
              Underwear & 117958 &  24.6 &  7.8 &  2 & 19 &  23 &  28 &  231 \\
                   Nail & 136649 &  24.7 & 15.3 &  2 & 16 &  22 &  28 &  265 \\
                   Star & 132814 &  24.8 &  6.8 &  2 & 20 &  24 &  28 &  295 \\
           Diving Board & 268348 &  25 & 16 &  2 & 14 &  22 &  32 &  784 \\
                    Axe & 115536 &  25.1 &  9.2 &  2 & 19 &  24 &  29 &  284 \\
                   Rake & 132704 &  25.2 & 11.7 &  2 & 18 &  22 &  30 &  200 \\
                 Circle & 118808 &  25.3 &  4.6 &  2 & 23 &  25 &  27 &  277 \\
                  Pants & 138311 &  25.4 &  7.1 &  2 & 21 &  24 &  29 &  269 \\
                    Hat & 200660 &  25.5 &  9.4 &  2 & 19 &  25 &  31 &  201 \\
                 Marker & 297232 &  25.6 & 14.3 &  2 & 17 &  22 &  30 &  516 \\
           Baseball Bat & 115325 &  25.7 &  7.5 &  2 & 21 &  25 &  28 &  213 \\
               Popsicle & 121696 &  25.7 &  9.2 &  2 & 21 &  24 &  28 &  397 \\
                 Pencil & 110089 &  25.9 & 11.4 &  2 & 18 &  23 &  31 &  163 \\
              Boomerang & 135561 &  26.1 &  6.9 &  2 & 22 &  26 &  29 &  251 \\
                  River & 126842 &  26.1 & 13 &  2 & 18 &  23 &  31 &  176 \\
                 Shovel & 112570 &  26.5 &  9.3 &  2 & 20 &  25 &  31 &  193 \\
             Floor Lamp & 144425 &  26.7 & 10.2 &  2 & 20 &  25 &  32 &  236 \\
                  Sword & 117275 &  26.7 &  9.1 &  2 & 21 &  26 &  31 &  396 \\
                 Shorts & 121009 &  26.8 &  8.2 &  2 & 21 &  25 &  30 &  148 \\
                Rainbow & 125254 &  27 & 17.8 &  2 & 16 &  23 &  31 &  284 \\
       The Eiffel Tower & 130433 &  27.2 & 12.1 &  2 & 19 &  25 &  33 &  312 \\
                  House & 132383 &  27.4 & 10.2 &  2 & 21 &  25 &  31 &  202 \\
            Screwdriver & 102453 &  27.6 &  9.9 &  2 & 21 &  26 &  32 &  226 \\
             Paper Clip & 121390 &  27.7 &  7.1 &  2 & 23 &  27 &  31 &  292 \\
               Sailboat & 132270 &  27.7 &  7.9 &  2 & 23 &  26 &  31 &  162 \\
                 Banana & 286030 &  27.8 & 11.3 &  2 & 21 &  25 &  32 &  205 \\
                 Candle & 135206 &  27.8 &  9.4 &  2 & 22 &  26 &  32 &  191 \\
                  Bread & 116991 &  27.9 & 10.7 &  2 & 22 &  26 &  31 &  393 \\
                   Pear & 114474 &  28 &  5.7 &  2 & 25 &  28 &  31 &  186 \\
                 Crayon & 119890 &  28.1 & 15.6 &  2 & 18 &  24 &  34 &  251 \\
                 Eraser &  96379 &  28.1 & 16.6 &  2 & 20 &  25 &  31 &  395 \\
                T-Shirt & 120847 &  28.2 &  6.2 &  2 & 24 &  28 &  32 &  109 \\
                  Anvil & 117463 &  28.3 &  8.2 &  2 & 23 &  28 &  33 &  217 \\
                   Sock & 188755 &  28.4 &  7.5 &  2 & 24 &  27 &  32 &  180 \\
                    Ear & 116811 &  28.5 &  9.8 &  2 & 22 &  27 &  34 &  222 \\
                Syringe & 113904 &  28.6 &  9.7 &  2 & 22 &  27 &  34 &  179 \\
                Mailbox & 124664 &  28.6 & 10.2 &  2 & 22 &  27 &  34 &  154 \\
               Postcard & 117710 &  29.3 & 10.8 &  2 & 22 &  28 &  35 &  281 \\
                   Foot & 181129 &  29.5 & 10 &  2 & 23 &  28 &  35 &  213 \\
              Hourglass & 128761 &  29.6 & 11.5 &  2 & 22 &  27 &  35 &  192 \\
               Squiggle & 109129 &  29.9 & 24.9 &  2 & 17 &  23 &  34 &  648 \\
                   Shoe & 115749 &  29.9 & 11.5 &  2 & 22 &  27 &  35 &  272 \\
                 Potato & 307270 &  29.9 &  9 &  2 & 23 &  28 &  35 &  233 \\
                 Church & 142273 &  30.1 & 11.8 &  2 & 22 &  28 &  36 &  133 \\
                Matches & 122008 &  30.1 & 19.9 &  2 & 16 &  24 &  38 &  274 \\
              Moustache & 163541 &  30.2 & 20.8 &  2 & 20 &  26 &  33 &  493 \\
             Toothpaste & 123825 &  30.6 & 13.5 &  2 & 22 &  27 &  36 &  169 \\
                 Bridge & 121181 &  30.6 & 11.7 &  2 & 22 &  29 &  37 &  175 \\
                  Tooth & 114696 &  30.8 &  9.1 &  2 & 25 &  30 &  34 &  236 \\
             Wine Glass & 124895 &  31 &  9.2 &  2 & 25 &  30 &  36 &  230 \\
                  Fence & 124669 &  31.1 & 13.5 &  2 & 22 &  29 &  38 &  199 \\
                  Crown & 129797 &  31.3 & 11.9 &  2 & 24 &  29 &  36 &  245 \\
             Toothbrush & 118514 &  31.3 & 18.4 &  2 & 18 &  28 &  41 &  229 \\
                   Jail & 115576 &  31.4 & 14.3 &  2 & 22 &  29 &  37 &  202 \\
                 Peanut & 122046 &  31.6 & 10.2 &  2 & 26 &  29 &  34 &  221 \\
                  Drill & 114826 &  31.9 &  9.7 &  2 & 25 &  30 &  37 &  174 \\
                   Fish & 126420 &  32 &  9.7 &  2 & 25 &  30 &  37 &  177 \\
              Snowflake & 113282 &  32.1 & 20.8 &  2 & 19 &  24 &  39 &  417 \\
             Waterslide & 163399 &  32.1 & 18.1 &  2 & 19 &  28 &  41 &  234 \\
               Lollipop & 124443 &  32.3 & 15.6 &  2 & 21 &  27 &  40 &  475 \\
                Sweater & 116097 &  32.7 &  9.8 &  2 & 26 &  31 &  37 &  196 \\
                    Bed & 107025 &  32.7 & 15 &  2 & 22 &  30 &  41 &  199 \\
                  Snake & 115263 &  32.8 & 10.4 &  2 & 26 &  32 &  38 &  205 \\
             Frying Pan & 117113 &  33 & 11.1 &  2 & 25 &  30 &  39 &  216 \\
               Mushroom & 136955 &  33 & 11.6 &  2 & 26 &  30 &  36 &  369 \\
                 Hammer & 111369 &  33 & 11.8 &  2 & 26 &  31 &  38 &  465 \\
                Feather & 113472 &  33.2 & 17.8 &  2 & 21 &  29 &  40 &  274 \\
                   Moon & 114803 &  33.5 & 22.5 &  2 & 23 &  27 &  33 &  584 \\
               Umbrella & 120514 &  33.5 & 11 &  2 & 25 &  32 &  40 &  328 \\
                Dolphin & 110335 &  33.6 &  8.9 &  2 & 27 &  32 &  38 &  244 \\
                  Grass & 119986 &  33.7 & 15.4 &  2 & 24 &  31 &  40 &  566 \\
                   Leaf & 116425 &  33.7 &  9.9 &  2 & 27 &  32 &  39 &  149 \\
              Megaphone & 121056 &  33.8 &  9.9 &  2 & 27 &  32 &  39 &  168 \\
                    Arm & 112701 &  33.9 &  8.7 &  2 & 28 &  33 &  39 &  187 \\
                 Bucket & 121530 &  33.9 &  8.9 &  2 & 28 &  33 &  39 &  340 \\
                   Vase & 123448 &  34 & 13.2 &  2 & 26 &  31 &  38 &  212 \\
               Dumbbell & 136063 &  34.1 & 16 &  2 & 27 &  32 &  38 &  444 \\
                   Belt & 169171 &  34.2 & 16.4 &  2 & 22 &  31 &  44 & 1025 \\
                Lighter & 114364 &  34.4 &  9.9 &  2 & 28 &  33 &  39 &  261 \\
                 Bowtie & 123949 &  34.4 & 12.4 &  2 & 27 &  33 &  39 &  406 \\
                Bandage & 125673 &  34.6 & 14.6 &  2 & 26 &  31 &  39 & 1176 \\
                   Barn & 129192 &  34.7 &  9.8 &  2 & 28 &  33 &  40 &  428 \\
                  Shark & 119434 &  34.9 & 11.7 &  2 & 26 &  33 &  41 &  172 \\
                  Broom & 113183 &  34.9 & 22 &  2 & 18 &  32 &  47 &  418 \\
              Ice Cream & 119837 &  35 & 13 &  2 & 26 &  32 &  41 &  360 \\
                    Cup & 121166 &  35 & 11.8 &  2 & 27 &  33 &  40 &  274 \\
                   Pond & 110628 &  35 & 14 &  2 & 25 &  32 &  42 &  227 \\
                    Toe & 131712 &  35.1 & 12.9 &  2 & 27 &  32 &  41 &  189 \\
             Flashlight & 217807 &  35.2 &  9.9 &  2 & 28 &  34 &  40 &  178 \\
                Bathtub & 152387 &  35.5 & 13.8 &  2 & 26 &  32 &  41 &  362 \\
                  Mouth & 126033 &  35.6 & 15 &  2 & 26 &  32 &  41 &  379 \\
                  Apple & 139902 &  35.7 &  7.5 &  2 & 31 &  35 &  40 &  190 \\
            Cruise Ship & 112147 &  35.8 & 16.8 &  2 & 25 &  31 &  41 &  255 \\
             Skateboard & 125552 &  35.9 & 10.7 &  2 & 29 &  35 &  41 &  237 \\
               Airplane & 135823 &  36.1 &  9.8 &  2 & 30 &  35 &  41 &  215 \\
                 Castle & 116690 &  36.3 & 11.9 &  2 & 28 &  34 &  43 &  153 \\
             Eyeglasses & 203817 &  36.4 &  9.5 &  2 & 31 &  36 &  40 &  466 \\
          Flying Saucer & 130045 &  36.4 & 14.6 &  2 & 27 &  33 &  42 &  272 \\
                    Saw & 112736 &  36.5 & 11.6 &  2 & 29 &  35 &  42 &  214 \\
                 Pliers & 150689 &  36.5 & 14.4 &  2 & 27 &  35 &  43 &  333 \\
               Clarinet & 117773 &  37 & 17 &  2 & 25 &  34 &  45 &  428 \\
             Light Bulb & 115279 &  37 & 12.1 &  2 & 28 &  34 &  43 &  212 \\
                Trumpet & 147595 &  37.1 & 16 &  2 & 26 &  34 &  44 &  355 \\
              Microwave & 123920 &  37.1 & 14 &  2 & 27 &  34 &  44 &  184 \\
The Great Wall Of China & 171064 &  37.2 & 36.8 &  2 & 20 &  28 &  41 &  812 \\
              Speedboat & 166626 &  37.3 & 12.9 &  2 & 28 &  35 &  44 &  173 \\
                 Helmet & 115185 &  37.3 & 15.6 &  2 & 28 &  34 &  42 &  461 \\
                  Purse & 112698 &  37.4 & 11.9 &  2 & 29 &  35 &  43 &  195 \\
        Hot Air Balloon & 121380 &  37.4 &  9.3 &  2 & 31 &  36 &  41 &  192 \\
          Picture Frame & 117673 &  37.4 & 14.7 &  2 & 28 &  34 &  42 &  294 \\
                 Jacket & 194143 &  37.7 & 11.2 &  2 & 30 &  36 &  44 &  254 \\
           Sleeping Bag & 100819 &  37.8 & 13.8 &  2 & 29 &  35 &  44 &  259 \\
                 Carrot & 125462 &  37.8 & 13.4 &  2 & 29 &  36 &  44 &  273 \\
       Aircraft Carrier &  94582 &  37.8 & 17.1 &  2 & 26 &  35 &  46 &  404 \\
                 Laptop & 239527 &  38.5 & 18.9 &  2 & 25 &  33 &  48 &  252 \\
                    Key & 139010 &  38.7 & 10.2 &  2 & 32 &  38 &  44 &  245 \\
              Submarine & 114889 &  38.7 & 15.9 &  2 & 27 &  34 &  47 &  231 \\
                    Mug & 140649 &  38.8 & 11.9 &  2 & 31 &  38 &  44 &  801 \\
                 Cooler & 249546 &  38.8 & 20.2 &  2 & 26 &  33 &  46 &  456 \\
             Dishwasher & 147814 &  39 & 23.5 &  2 & 25 &  32 &  44 &  460 \\
         Roller Coaster & 121602 &  39.1 & 17.2 &  2 & 27 &  36 &  48 &  367 \\
             Television & 117704 &  39.1 & 13.3 &  2 & 30 &  37 &  45 &  201 \\
                Hot Dog & 160034 &  39.1 & 12.9 &  2 & 30 &  37 &  45 &  202 \\
                  Mouse & 166197 &  39.4 & 15.3 &  2 & 29 &  36 &  47 &  309 \\
            Garden Hose & 116044 &  39.4 & 25.7 &  2 & 20 &  33 &  53 &  650 \\
                  Clock & 118643 &  39.5 & 10.2 &  2 & 32 &  38 &  44 &  201 \\
            Spreadsheet & 148297 &  39.5 & 20.9 &  2 & 29 &  36 &  45 &  550 \\
              Asparagus & 146218 &  39.7 & 21.6 &  2 & 25 &  34 &  48 &  665 \\
       Animal Migration & 115949 &  39.8 & 20.3 &  2 & 25 &  35 &  49 &  243 \\
                 Camera & 124706 &  39.8 & 10.8 &  2 & 33 &  38 &  45 &  213 \\
             Flip Flops & 112705 &  39.9 & 12.8 &  2 & 30 &  38 &  48 &  240 \\
                   Harp & 263523 &  40.1 & 13.2 &  2 & 31 &  38 &  47 &  382 \\
               Flamingo & 116251 &  40.2 & 11.1 &  2 & 33 &  39 &  46 &  223 \\
                   Pool & 127961 &  40.3 & 20.3 &  2 & 26 &  37 &  50 &  562 \\
                   Swan & 132994 &  40.5 & 11.8 &  2 & 32 &  38 &  46 &  178 \\
             Lighthouse & 138953 &  40.8 & 12.9 &  2 & 32 &  39 &  48 &  225 \\
            Stethoscope & 131906 &  40.9 & 14 &  2 & 32 &  38 &  47 &  259 \\
              Crocodile & 106410 &  40.9 & 13.5 &  2 & 31 &  39 &  48 &  170 \\
                  Piano & 114011 &  41 & 15.7 &  2 & 30 &  38 &  48 &  308 \\
               Hospital & 145485 &  41 & 15.7 &  2 & 30 &  38 &  48 &  224 \\
              Saxophone & 109632 &  41.2 & 12.6 &  2 & 33 &  39 &  46 &  345 \\
             Cell Phone & 113164 &  41.2 & 15.2 &  2 & 31 &  38 &  47 &  205 \\
                   Oven & 192471 &  41.3 & 16.8 &  2 & 30 &  37 &  49 &  280 \\
                  Beach & 115542 &  41.3 & 18.6 &  2 & 28 &  38 &  50 &  276 \\
                 Cactus & 125063 &  41.4 & 13.5 &  2 & 33 &  39 &  46 &  201 \\
               Computer & 117485 &  41.5 & 15.6 &  2 & 30 &  39 &  50 &  263 \\
         Remote Control & 112246 &  41.5 & 18 &  2 & 29 &  38 &  50 &  268 \\
                   Yoga & 258493 &  41.6 & 16.6 &  2 & 30 &  38 &  49 &  329 \\
                Dresser & 101460 &  41.6 & 14.6 &  2 & 31 &  39 &  49 &  188 \\
                   Hand & 269836 &  41.7 &  8.2 &  2 & 37 &  41 &  46 &  307 \\
            Smiley Face & 119479 &  41.7 & 15.5 &  2 & 35 &  40 &  48 &  456 \\
                Toaster & 102566 &  41.8 & 12.8 &  2 & 33 &  40 &  48 &  199 \\
                    Sun & 129631 &  41.8 & 12.2 &  2 & 34 &  39 &  46 &  292 \\
             Watermelon & 124482 &  42.2 & 19.3 &  2 & 29 &  40 &  51 &  359 \\
                   Book & 111206 &  42.2 & 14.9 &  2 & 32 &  40 &  50 &  261 \\
                  Steak & 109136 &  42.5 & 16.1 &  2 & 31 &  40 &  50 &  282 \\
           Fire Hydrant & 115295 &  42.6 & 14.5 &  2 & 32 &  40 &  50 &  196 \\
              Bottlecap & 131267 &  42.7 & 17.6 &  2 & 31 &  39 &  50 &  379 \\
               Trombone & 162833 &  42.8 & 16.1 &  2 & 32 &  40 &  50 &  308 \\
              Parachute & 120419 &  42.9 & 13.6 &  2 & 33 &  41 &  50 &  222 \\
                  Couch & 111978 &  43 & 13.3 &  2 & 34 &  41 &  50 &  241 \\
               Baseball & 126439 &  43.1 &  9.4 &  2 & 37 &  42 &  48 &  344 \\
                   Rain & 130678 &  43.1 & 23.3 &  2 & 23 &  42 &  58 &  322 \\
          Birthday Cake & 137263 &  43.2 & 15.2 &  2 & 33 &  41 &  50 &  328 \\
              Paint Can & 110475 &  43.2 & 15.5 &  2 & 33 &  40 &  50 &  303 \\
                Giraffe & 122396 &  43.4 & 14.5 &  2 & 34 &  41 &  50 &  215 \\
                 Toilet & 125045 &  43.5 & 11.3 &  2 & 36 &  43 &  50 &  165 \\
           Power Outlet & 147542 &  43.6 & 14 &  2 & 34 &  42 &  52 &  257 \\
             Headphones & 114762 &  43.8 & 16.3 &  2 & 35 &  41 &  48 &  397 \\
           Pickup Truck & 115813 &  43.9 & 17.4 &  2 & 32 &  41 &  51 &  225 \\
             Coffee Cup & 161463 &  44.1 & 12.7 &  2 & 36 &  43 &  50 &  280 \\
                  Cloud & 117587 &  44.5 & 13.5 &  2 & 36 &  43 &  50 &  333 \\
                  Camel & 115454 &  44.7 & 11.2 &  2 & 37 &  44 &  51 &  161 \\
             Wristwatch & 140672 &  44.7 & 16.5 &  2 & 33 &  41 &  54 &  366 \\
            Hockey Puck & 181363 &  44.9 & 50.6 &  2 & 27 &  33 &  41 & 2644 \\
                 Violin & 195300 &  45.2 & 14.1 &  2 & 35 &  43 &  52 &  256 \\
                  Whale & 109081 &  45.2 & 13.3 &  2 & 36 &  43 &  52 &  202 \\
                 Teapot & 120110 &  45.3 & 10.1 &  2 & 38 &  44 &  51 &  222 \\
                Snorkel & 132616 &  45.3 & 14.6 &  2 & 35 &  43 &  54 &  208 \\
               Necklace & 112929 &  45.3 & 33 &  2 & 24 &  33 &  55 &  398 \\
               Passport & 128317 &  45.6 & 16.1 &  2 & 34 &  43 &  54 &  196 \\
              Stop Sign & 114746 &  45.8 & 12 &  2 & 38 &  46 &  54 &  270 \\
                Snowman & 323952 &  46.1 &  9 &  2 & 40 &  46 &  51 &  179 \\
                   Bird & 111611 &  46.2 & 16.6 &  2 & 36 &  46 &  56 &  185 \\
             Chandelier & 145602 &  46.3 & 21.1 &  2 & 32 &  42 &  56 &  445 \\
                  Donut & 137038 &  46.3 & 11.4 &  2 & 39 &  44 &  51 &  236 \\
             Rhinoceros & 166539 &  46.5 & 12 &  2 & 38 &  45 &  53 &  178 \\
             Microphone & 113497 &  46.8 & 19.8 &  2 & 35 &  44 &  53 &  396 \\
          Traffic Light & 119687 &  47.1 & 11.7 &  2 & 40 &  47 &  54 &  262 \\
               Scissors & 111293 &  47.2 & 15.4 &  2 & 36 &  44 &  56 &  269 \\
               Windmill & 114242 &  47.2 & 15.1 &  2 & 37 &  45 &  55 &  264 \\
              Palm Tree & 116984 &  47.7 & 17.7 &  2 & 36 &  44 &  55 &  247 \\
                   Duck & 113764 &  47.9 & 12.7 &  2 & 39 &  46 &  55 &  135 \\
        Washing Machine & 116488 &  48 & 17.3 &  2 & 37 &  44 &  54 &  433 \\
            Ceiling Fan & 108077 &  48 & 16 &  2 & 38 &  46 &  56 &  299 \\
                Lantern & 127958 &  48 & 13.7 &  2 & 39 &  46 &  55 &  205 \\
                 Cannon & 119439 &  48 & 17.2 &  2 & 37 &  45 &  55 &  460 \\
                    Map & 112151 &  48.2 & 17.7 &  2 & 35 &  45 &  58 &  243 \\
                  Radio & 128562 &  48.3 & 20.2 &  2 & 35 &  46 &  58 &  426 \\
                  Cello & 127820 &  48.3 & 14.1 &  2 & 39 &  47 &  56 &  370 \\
                    Van & 143947 &  48.6 & 15 &  2 & 39 &  46 &  55 &  222 \\
                    Bat &  96152 &  48.6 & 14 &  2 & 39 &  47 &  55 &  388 \\
                Compass & 120919 &  48.6 & 13.3 &  2 & 39 &  46 &  57 &  205 \\
                  Truck & 122580 &  48.7 & 13.8 &  2 & 39 &  47 &  56 &  244 \\
              Telephone & 111275 &  48.8 & 20.1 &  2 & 34 &  45 &  59 &  227 \\
              Hamburger & 123908 &  49.3 & 16 &  2 & 38 &  46 &  57 &  304 \\
             Basketball & 126373 &  49.7 &  9.9 &  2 & 44 &  49 &  54 &  239 \\
                 Parrot & 163567 &  50 & 15.9 &  2 & 39 &  47 &  58 &  217 \\
            House Plant & 116752 &  50.1 & 17.5 &  2 & 38 &  47 &  58 &  274 \\
         Tennis Racquet & 209236 &  50.3 & 13.2 &  2 & 42 &  49 &  57 &  415 \\
              Blueberry & 112237 &  50.4 & 32.3 &  2 & 34 &  42 &  54 &  551 \\
               Sandwich & 116583 &  50.4 & 17.6 &  2 & 38 &  47 &  59 &  291 \\
                Hot Tub &  98344 &  50.6 & 21.2 &  2 & 35 &  47 &  62 &  276 \\
             Police Car & 122792 &  50.9 & 17.9 &  2 & 38 &  49 &  61 &  237 \\
                    Car & 160789 &  51 & 14.7 &  2 & 41 &  49 &  58 &  265 \\
             Paintbrush & 165044 &  51.2 & 20.2 &  2 & 38 &  48 &  61 &  381 \\
               Backpack & 118110 &  51.3 & 14.3 &  2 & 42 &  49 &  59 &  296 \\
             Helicopter & 137966 &  51.6 & 16.7 &  2 & 40 &  49 &  60 &  350 \\
             Calculator & 120487 &  51.7 & 17.9 &  2 & 39 &  48 &  61 &  229 \\
             Strawberry & 118562 &  51.9 & 16.4 &  2 & 41 &  49 &  59 &  285 \\
              Pineapple & 121938 &  52.1 & 17.9 &  2 & 40 &  48 &  60 &  286 \\
                    Eye & 121030 &  52.1 & 24.2 &  2 & 37 &  46 &  60 &  457 \\
               Mosquito & 116609 &  52.1 & 18.7 &  2 & 40 &  49 &  60 &  371 \\
                 Basket & 108534 &  52.7 & 19.3 &  2 & 40 &  50 &  62 &  458 \\
                  Drums & 115333 &  53.1 & 15.8 &  2 & 42 &  50 &  61 &  547 \\
                 Spider & 187865 &  53.2 & 22.8 &  2 & 41 &  49 &  58 &  523 \\
                   Cake & 111861 &  53.2 & 18.9 &  2 & 40 &  50 &  62 &  295 \\
                 Guitar & 111775 &  53.4 & 14.3 &  2 & 44 &  51 &  60 &  253 \\
                Octopus & 143558 &  53.5 & 14.6 &  2 & 44 &  52 &  61 &  292 \\
                   Sink & 186455 &  53.8 & 16.3 &  2 & 42 &  51 &  62 &  260 \\
                 Stereo & 109566 &  53.9 & 18.1 &  2 & 42 &  51 &  62 &  272 \\
                  Onion & 122741 &  54.1 & 24.1 &  2 & 40 &  50 &  63 &  550 \\
               Calendar & 300070 &  54.1 & 19.4 &  2 & 41 &  50 &  64 &  299 \\
             Binoculars & 108734 &  54.5 & 13.3 &  2 & 46 &  52 &  60 &  300 \\
               Kangaroo & 152511 &  54.9 & 15.5 &  2 & 44 &  53 &  64 &  366 \\
                  Snail & 128512 &  55.2 & 15.5 &  2 & 46 &  53 &  62 &  479 \\
                Penguin & 231826 &  55.2 & 16 &  2 & 44 &  53 &  64 &  311 \\
                  Wheel & 129765 &  55.2 & 15 &  2 & 45 &  53 &  62 &  368 \\
           Rollerskates & 114927 &  55.3 & 14.9 &  2 & 45 &  53 &  63 &  367 \\
              Butterfly & 114549 &  55.6 & 11.6 &  2 & 48 &  54 &  61 &  247 \\
              Fireplace & 133604 &  55.6 & 19.4 &  2 & 42 &  52 &  65 &  270 \\
                Bicycle & 122540 &  55.8 & 15.1 &  3 & 45 &  53 &  63 &  263 \\
                    Ant & 115718 &  56 & 21.8 &  2 & 45 &  53 &  62 &  597 \\
               Elephant & 104986 &  56.6 & 14.4 &  2 & 46 &  55 &  65 &  172 \\
              Firetruck & 198756 &  56.7 & 18.6 &  2 & 44 &  54 &  66 &  246 \\
                Tractor & 105016 &  57 & 17.4 &  2 & 47 &  53 &  63 &  366 \\
                   Face & 148436 &  57.1 & 19 &  2 & 45 &  54 &  65 &  310 \\
                   Tree & 138514 &  57.3 & 34.8 &  2 & 40 &  48 &  60 &  580 \\
                  Horse & 156302 &  57.6 & 20.2 &  2 & 43 &  54 &  68 &  679 \\
              Motorbike & 148627 &  57.9 & 22.4 &  2 & 44 &  52 &  64 &  702 \\
                    Bus & 144234 &  58 & 17.1 &  2 & 46 &  56 &  68 &  229 \\
                    Cat & 103031 &  58.3 & 14.6 &  2 & 48 &  56 &  67 &  175 \\
              Bulldozer & 165474 &  58.4 & 16.9 &  2 & 47 &  56 &  67 &  267 \\
            Alarm Clock & 113911 &  58.6 & 16.4 &  2 & 47 &  56 &  67 &  218 \\
              Ambulance & 134474 &  59.5 & 17.7 &  2 & 48 &  57 &  68 &  252 \\
                   Bush & 111324 &  60.6 & 47.7 &  2 & 37 &  46 &  63 &  658 \\
             Sea Turtle & 110218 &  60.6 & 17.5 &  2 & 49 &  58 &  69 &  341 \\
                    Dog & 143285 &  60.8 & 19.3 &  2 & 48 &  58 &  71 &  786 \\
                  Skull & 119276 &  60.9 & 17.7 &  2 & 50 &  58 &  68 &  385 \\
                 Flower & 138836 &  61 & 16.2 &  2 & 50 &  60 &  70 &  353 \\
                 Cookie & 126590 &  61.3 & 18 &  2 & 49 &  58 &  70 &  283 \\
                   Frog & 145286 &  61.5 & 18.2 &  2 & 49 &  59 &  71 &  360 \\
                   Bear & 127671 &  61.9 & 21.6 &  2 & 48 &  58 &  72 &  614 \\
                 Dragon & 115480 &  62.3 & 17.8 &  2 & 50 &  60 &  72 &  280 \\
                   Crab & 106466 &  62.8 & 14.9 &  2 & 52 &  61 &  71 &  234 \\
          The Mona Lisa & 111580 &  63 & 20.1 &  2 & 49 &  59 &  73 &  332 \\
                 Rabbit & 133323 &  63 & 15.3 &  2 & 53 &  61 &  71 &  526 \\
               Campfire & 125085 &  63.1 & 24.1 &  2 & 47 &  58 &  73 &  370 \\
             School Bus & 116094 &  63.3 & 23.4 &  2 & 46 &  62 &  78 &  240 \\
                Lobster & 118228 &  64.5 & 17.1 &  2 & 53 &  62 &  73 &  459 \\
               Scorpion & 143724 &  64.8 & 18.4 &  2 & 53 &  62 &  74 &  331 \\
                Mermaid & 158345 &  66 & 16.5 &  2 & 54 &  64 &  75 &  199 \\
                  Zebra & 127159 &  66.1 & 17.5 &  2 & 54 &  64 &  75 &  325 \\
                 Garden & 139572 &  66.2 & 26.4 &  2 & 48 &  63 &  81 &  710 \\
                    Bee & 110906 &  66.4 & 16.2 &  2 & 55 &  64 &  74 &  225 \\
                  Train & 113521 &  66.6 & 24.7 &  2 & 49 &  64 &  81 &  334 \\
                  Pizza & 124422 &  66.6 & 21.8 &  2 & 51 &  62 &  78 &  277 \\
                  Angel & 127756 &  68 & 16.2 &  2 & 57 &  66 &  77 &  248 \\
               Squirrel & 134923 &  68.8 & 21 &  2 & 55 &  65 &  77 &  347 \\
                    Owl & 147654 &  69.1 & 18.4 &  2 & 57 &  67 &  79 &  255 \\
                 Goatee & 168087 &  69.3 & 26 &  2 & 52 &  64 &  81 & 1109 \\
                   Peas & 139784 &  69.3 & 30.9 &  2 & 51 &  63 &  80 & 3712 \\
                  Sheep & 117555 &  69.4 & 27.2 &  2 & 53 &  63 &  77 &  450 \\
                    Fan & 114194 &  70.5 & 18.4 &  2 & 58 &  68 &  80 &  464 \\
                    Pig & 164788 &  72.5 & 17.1 &  2 & 61 &  70 &  82 &  242 \\
               Bracelet & 108207 &  73.8 & 34.5 &  2 & 46 &  67 &  96 &  462 \\
                  Stove &  94584 &  74.5 & 22.8 &  2 & 60 &  71 &  84 &  457 \\
                  Tiger & 110177 &  77.5 & 27.2 &  2 & 61 &  74 &  89 &  778 \\
             Teddy-Bear & 157583 &  78.5 & 19.3 &  2 & 65 &  77 &  90 &  246 \\
                 Monkey & 105650 &  78.7 & 19.5 &  2 & 65 &  77 &  90 &  237 \\
            Soccer Ball & 119239 &  79.3 & 40 &  2 & 55 &  67 &  89 & 1227 \\
               Hedgehog & 103226 &  79.5 & 26.9 &  2 & 61 &  74 &  93 &  444 \\
               Broccoli & 126608 &  81.8 & 42.8 &  2 & 50 &  70 & 103 &  535 \\
                  Brain & 126282 &  82.4 & 37.4 &  2 & 59 &  75 &  97 &  575 \\
                   Lion &  98976 &  82.6 & 22.5 &  2 & 67 &  79 &  94 &  369 \\
                Raccoon & 101174 &  85 & 35.4 &  2 & 63 &  78 &  99 &  742 \\
                    Cow & 101099 &  85.1 & 30.5 &  2 & 63 &  79 & 101 &  375 \\
                  Beard & 146100 &  87.5 & 41.2 &  2 & 60 &  79 & 106 &  590 \\
                 Grapes & 143320 &  87.9 & 28.1 &  2 & 69 &  85 & 104 &  374 \\
                Tornado & 138504 &  92.4 & 47.2 &  2 & 61 &  82 & 113 &  730 \\
              Hurricane & 130236 &  97.7 & 45.2 &  2 & 66 &  89 & 121 &  690 \\
             Camouflage & 150936 & 101 & 54.8 &  2 & 68 &  88 & 118 & 1001 \\
                  Panda &  94814 & 102.7 & 39.2 &  2 & 75 &  94 & 120 &  646 \\
             Blackberry & 113736 & 126.8 & 63.4 &  2 & 85 & 117 & 156 &  911 \\
\end{longtable}


==> tables/correlation_accuracy_prior.tex <==
\begin{table}
\centering
\caption{Correlation between Accuracy and Prior}
\label{tab:correlation_accuracy_prior}
\begin{tabular}{lrrrr}
\toprule
{} &  Coordinates &  Images &  Prior & Complexity \\
\midrule
\textbf{Coordinates} &         1.00 &    0.49 &   0.19 &       -0.28 \\
\textbf{Images     } &         0.49 &    1.00 &   0.15 &       -0.13 \\
\textbf{Prior      } &         0.19 &    0.15 &   1.00 &       -0.05 \\
\textbf{Complexity } &        -0.28 &   -0.13 &  -0.05 &        1.00 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Correlation between Accuracy and Prior (only original)}
\label{tab:correlation_accuracy_prior}
\begin{tabular}{lrrrr}
\toprule
{} &  Coordinates &  Images &  Prior & Complexity \\
\midrule
\textbf{Coordinates} &         1.00 &    0.41 &   0.22 &       -0.31 \\
\textbf{Images     } &         0.41 &    1.00 &   0.21 &       -0.27 \\
\textbf{Prior      } &         0.22 &    0.21 &   1.00 &       -0.05 \\
\textbf{Complexity } &        -0.31 &   -0.27 &  -0.05 &        1.00 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}
\centering
\caption{Correlation between Accuracy and Prior (only simplified)}
\label{tab:correlation_accuracy_prior}
\begin{tabular}{lrrrr}
\toprule
{} &  Coordinates &  Images &  Prior & Complexity \\
\midrule
\textbf{Coordinates} &         1.00 &    0.49 &   0.18 &       -0.28 \\
\textbf{Images     } &         0.49 &    1.00 &   0.14 &       -0.12 \\
\textbf{prior      } &         0.18 &    0.14 &   1.00 &       -0.05 \\
\textbf{Complexity } &        -0.28 &   -0.12 &  -0.05 &        1.00 \\
\bottomrule
\end{tabular}
\end{table}



==> tables/dificulty.tex <==
\begin{table}
\centering
\caption{Number of segments per concept}
\label{table:complexity}
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrr}
\toprule
{} & No. of Segments Sample(avg. $\pm$ std.) &  Prior & No. of Segments Dataset (avg. $\pm$ std.) \\
Concept  &                          &        &                           \\
\midrule
train    &            $66.88\pm14.86$ &     64 &             $69.22\pm23.25$ \\
horse    &            $52.76\pm11.96$ &     32 &             $56.85\pm19.44$ \\
car      &              $52.0\pm8.34$ &     72 &             $54.34\pm14.06$ \\
cat      &              $49.46\pm8.8$ &     21 &              $52.8\pm13.17$ \\
tree     &             $46.75\pm8.94$ &     50 &             $57.94\pm36.15$ \\
hand     &             $42.97\pm5.49$ &     46 &               $43.19\pm7.9$ \\
map      &            $41.41\pm12.45$ &     51 &              $45.49\pm17.9$ \\
airplane &             $34.28\pm5.84$ &     12 &              $36.03\pm9.33$ \\
rain     &            $32.59\pm18.56$ &      8 &             $36.39\pm23.14$ \\
fish     &              $31.2\pm5.38$ &     80 &              $33.86\pm9.37$ \\
ear      &             $28.78\pm6.73$ &     66 &                $30.2\pm9.8$ \\
envelope &             $24.57\pm3.99$ &     10 &              $25.96\pm6.81$ \\
star     &             $24.12\pm3.79$ &     43 &              $25.18\pm6.86$ \\
house    &             $23.97\pm5.13$ &     83 &               $25.98\pm9.1$ \\
chair    &             $20.39\pm8.28$ &     54 &             $22.49\pm10.67$ \\
square   &               $15.3\pm2.9$ &     40 &              $15.94\pm4.31$ \\
line     &              $9.39\pm3.99$ &     70 &              $11.65\pm7.66$ \\
\bottomrule
\end{tabular}
}
\end{table}

